Approximately Equivariant Recurrent Generative Models for Quasi-Periodic Time Series with a Progressive Training Scheme

We present a simple yet effective generative model for time series, based on a Recurrent Variational Autoencoder that we refer to as AEQ-RVAE-ST. Recurrent layers often struggle with unstable optimization and poor convergence when modeling long sequences. To address these limitations, we introduce a training scheme that subsequently increases the sequence length, stabilizing optimization and enabling consistent learning over extended horizons. By composing known components into a recurrent, approximately time-shift-equivariant topology, our model introduces an inductive bias that aligns with the structure of quasi-periodic and nearly stationary time series. Across several benchmark datasets, AEQ-RVAE-ST matches or surpasses state-of-the-art generative models, particularly on quasi-periodic data, while remaining competitive on more irregular signals. Performance is evaluated through ELBO, Fr\'echet Distance, discriminative metrics, and visualizations of the learned latent embeddings.

==> figures/tsne_sine.tex <==
\begin{figure}[ht]
\centering
\raisebox{-0.5\height}{\makebox[.8em][l]{\small\shortstack{\rvaect\\(ours)}}}
\hspace{1cm}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_ti-rvae_Sine_100.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_ti-rvae_Sine_300.jpg}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_ti-rvae_Sine_500.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_ti-rvae_Sine_1000.jpg}\\
\makebox[1.1em][l]{\small \timegan}%
\hspace{1cm}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timegan_Sine_100.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timegan_Sine_300.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timegan_Sine_500.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timegan_Sine_1000.jpg}\\
%\makebox[1.1em][l]{\small WaveGan}%
%\hspace{1cm}
%\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan_Sine_100.jpg}%\hspace{1pt}%
%\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan_Sine_300.jpg}%\hspace{1pt}%
%\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan_Sine_500.jpg}%\hspace{1pt}%
%\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan_Sine_1000.jpg}\\
\makebox[1.1em][l]{\small \wavegan}%
\hspace{1cm}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan2_Sine_100.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan2_Sine_300.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan2_Sine_500.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_wavegan2_Sine_1000.jpg}\\
\makebox[1.1em][l]{\small \timevae}%
\hspace{1cm}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timevae2_Sine_100.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timevae2_Sine_300.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timevae2_Sine_500.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_timevae2_Sine_1000.jpg}\\
\hspace{-1.2em}\makebox[1.9em][l]{\small\diffusionts}
\hspace{1cm}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_diffusion-ts_Sine_100.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_diffusion-ts_Sine_300.jpg}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_diffusion-ts_Sine_500.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_diffusion-ts_Sine_1000.jpg}\\
\hspace{-1.2em}\raisebox{-0.5\height}{\makebox[1.8em][l]{\small\shortstack{Time-\\Transformer}}}
%\makebox[1.4em][l]{\small %
\hspace{1cm}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_time-transformer_Sine_100.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_time-transformer_Sine_300.jpg}
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_time-transformer_Sine_500.jpg}%\hspace{1pt}%
\includegraphics[width=0.22\textwidth,valign=c]{images/pcatsne/pca_tsne_10.04/tsne_time-transformer_Sine_1000.jpg}\\
\vspace{.3cm}
\makebox[1.1em][l]{\small\hspace{-5cm}Sine, l=100\hspace{1.8cm}Sine, l=300\hspace{1.8cm}Sine, l=500\hspace{1.7cm}Sine, l=1000}%
\caption{t-SNE plots for all sequence lengths on the Sine dataset. At $l=100$, all models perform similarly well, except \timegan\ which consistently performs less effectively. From $l=500$ onward, \timetransformer\ also shows a decline in performance. \rvaect,\ \diffusionts,\ \wavegan\ and \timevae\ perform equally well throughout all sequence lengths. However, when looking at Figure \ref{fig:sine_comparison}, this does not fully reflect the models performance, as the limitations in accounting for temporal dependencies lead to significantly reduced effectiveness.}
\end{figure}
